Finite size scaling in Ising-like systems with quenched random fields: Evidence of hyperscaling violation

In systems belonging to the universality class of the random field Ising model, the standard hyperscaling relation between critical exponents does not hold, but is replaced by a modified hyperscaling relation. As a result, standard formulations of finite size scaling near critical points break down. In this work, the consequences of modified hyperscaling are analyzed in detail. The most striking outcome is that the free energy cost \Delta F of interface formation at the critical point is no longer a universal constant, but instead increases as a power law with system size, \Delta F proportional to $L^\theta$, with $\theta$ the violation of hyperscaling critical exponent, and L the linear extension of the system. This modified behavior facilitates a number of new numerical approaches that can be used to locate critical points in random field systems from finite size simulation data. We test and confirm the new approaches on two random field systems in three dimensions, namely the random field Ising model, and the demixing transition in the Widom-Rowlinson fluid with quenched obstacles.

==> Makefile <==
DOCUMENT  = bar0
CITEULIKE = mc1975
PASSWORD  = 

fast:
	latex $(DOCUMENT)

dvi:
	make clean
	latex $(DOCUMENT)
	latex $(DOCUMENT)
	latex $(DOCUMENT)

ps:
	make clean
	make dvi
	dvips $(DOCUMENT).dvi $(DOCUMENT).ps

pdf:	
	make pdffigs
	pdflatex $(DOCUMENT)
	pdflatex $(DOCUMENT)
	pdflatex $(DOCUMENT)
	pdflatex $(DOCUMENT)

bib:
	make sed
	make veryclean
	latex $(DOCUMENT)
	bibtex $(DOCUMENT)
	latex $(DOCUMENT)
	latex $(DOCUMENT)
	latex $(DOCUMENT)

view:
	xdvi -s 4 $(DOCUMENT) -browser firefox&

cul:
	make veryclean
	wget -O /dev/null --keep-session-cookies --save-cookies cookies.txt \
        --post-data="username=$(CITEULIKE)&password=$(PASSWORD)&perm=1" http://www.citeulike.org/login.do
	wget -O refs.bib --load-cookies cookies.txt http://www.citeulike.org/bibtex/user/$(CITEULIKE) 
	make bib

sed:
	sed -n -f JOURNAL_AB.sed < refs.bib > refs.bib.tmp
	mv refs.bib.tmp refs.bib

bibstyle:
	tex sfb.dbj

spell:
	aspell --mode=tex -c $(DOCUMENT).tex

pdffigs: $(patsubst %.eps,%.pdf,$(wildcard *.eps))

%.pdf : %.eps
	epstopdf $<

clean:
	rm -f *.aux *.log *.blg *.toc *.out *.fgx *.tbx *.lof *.lot \
              *.dvi *.idx *.ilg *.ind $(DOCUMENT).ps *.pdf *.end 

veryclean:
	make clean
	rm -f *.bbl

